SwiftLane: Towards Fast and Efficient Lane Detection

Recent work done on lane detection has been able to detect lanes accurately in complex scenarios, yet many fail to deliver real-time performance specifically with limited computational resources. In this work, we propose SwiftLane: a simple and light-weight, end-to-end deep learning based framework, coupled with the row-wise classification formulation for fast and efficient lane detection. This framework is supplemented with a false positive suppression algorithm and a curve fitting technique to further increase the accuracy. Our method achieves an inference speed of 411 frames per second, surpassing state-of-the-art in terms of speed while achieving comparable results in terms of accuracy on the popular CULane benchmark dataset. In addition, our proposed framework together with TensorRT optimization facilitates real-time lane detection on a Nvidia Jetson AGX Xavier as an embedded system while achieving a high inference speed of 56 frames per second.

==> LaneQualitativeResults/lane_results_images.tex <==

\begin{figure}[ht]
     \centering
     \begin{subfigure}[b]{0.32\linewidth}
         \centering
         \includegraphics[width=.95\linewidth]{LaneQualitativeResults/lane_images/1_lanes_highway.jpg}
         %\caption{Sub-cap 1.}
         %\label{sfi:sf1}
     \end{subfigure}%
     \begin{subfigure}[b]{0.32\linewidth}
         \centering
         \includegraphics[width=.95\linewidth]{LaneQualitativeResults/lane_images/4_lanes_rural.jpg}
         %\caption{Sub-cap2}
         %\label{sfi:sf2}
     \end{subfigure}%
     \begin{subfigure}[b]{0.32\linewidth}
         \centering
         \includegraphics[width=.95\linewidth]{LaneQualitativeResults/lane_images/3_lanes_urban.jpg}
         %\caption{Sub-cap 2}
         %\label{sfi:sf2}
     \end{subfigure}%
          \begin{subfigure}[b]{0.32\linewidth}
         \centering
         \includegraphics[width=.95\linewidth]{LaneQualitativeResults/lane_images/2_lanes_highway.jpg}
         %\caption{Sub-cap 2}
         %\label{sfi:sf2}
     \end{subfigure}%
     \vspace{0.5em}
     
         \begin{subfigure}[b]{0.32\linewidth}
         \centering
         \includegraphics[width=.95\linewidth]{LaneQualitativeResults/lane_images/5_lanes_rural.jpg}
         %\caption{Sub-cap 1.}
         %\label{sfi:sf1}
     \end{subfigure}%
     \begin{subfigure}[b]{0.32\linewidth}
         \centering
         \includegraphics[width=.95\linewidth]{LaneQualitativeResults/lane_images/6_lanes_fp.jpg}
         %\caption{Sub-cap2}
         %\label{sfi:sf2}
     \end{subfigure}%
     \begin{subfigure}[b]{0.32\linewidth}
         \centering
         \includegraphics[width=.95\linewidth]{LaneQualitativeResults/lane_images/7_lanes_fp.jpg}
         %\caption{Sub-cap 2}
         %\label{sfi:sf2}
     \end{subfigure}%
          \begin{subfigure}[b]{0.32\linewidth}
         \centering
         \includegraphics[width=.95\linewidth]{LaneQualitativeResults/lane_images/8_lanes_undetected.jpg}
         %\caption{Sub-cap 2}
         %\label{sfi:sf2}
     \end{subfigure}%
     \vspace{0.5em}
     
     \caption{ 
    Visualization of lane detection results}
     \label{fi:local_lane_qualitative_results}
%    \vspace{-5ex}
\end{figure}
